Longitudinal Self-Supervision for COVID-19 Pathology Quantification

Quantifying COVID-19 infection over time is an important task to manage the hospitalization of patients during a global pandemic. Recently, deep learning-based approaches have been proposed to help radiologists automatically quantify COVID-19 pathologies on longitudinal CT scans. However, the learning process of deep learning methods demands extensive training data to learn the complex characteristics of infected regions over longitudinal scans. It is challenging to collect a large-scale dataset, especially for longitudinal training. In this study, we want to address this problem by proposing a new self-supervised learning method to effectively train longitudinal networks for the quantification of COVID-19 infections. For this purpose, longitudinal self-supervision schemes are explored on clinical longitudinal COVID-19 CT scans. Experimental results show that the proposed method is effective, helping the model better exploit the semantics of longitudinal data and improve two COVID-19 quantification tasks.

==> temp/2.RelatedWork.tex <==
\section{Related Work} %from Cocos master thesis --> needs to be modified

\subsection{COVID-19 segmentation}

Since the outbreak of COVID-19, numerous studies have attempted to segment the disease \cite{Wang2020,Shan2021,Zhou2020,Fan2020} to allow assessment of severity and prediction of outcome.
However, segmentation of COVID-19 CTs is very challenging for several reasons. Firstly, the size, position, and shape of lesions vary during the course of the disease and between patients. Moreover, they have different textures and ambiguous boundaries \cite{Fan2020,Wang2020}. The second is, that there is often not enough labeled data to train a reliable deep model, as an expert is needed for the annotation \cite{Wang2020}, and also because many datasets are not freely available \cite{pseudo_lesion}. Third, the labeled data is often noisy due to the difficulty in delineating the lesions and a high inter- and intra-observer variability \cite{Wang2020}. However, the success of medical image segmentation depends on accurately labeled data. Some studies on the segmentation of COVID-19 have attempted to counteract these problems and are presented in the following.

Wang et al. \cite{Wang2020} addressed the problem of noisy labels by proposing a noise-resistant training method that is able to learn from inaccurate training labels. For this, they introduced a noise-robust Dice loss, which is a generalization of the Dice loss for segmentation and the mean absolute error (MAE). The results show that their noise-resistant Dice loss outperforms other noise-resistant loss functions and their model outperforms standard training and surpasses other noise-resistant training approaches for COVID-19 lesion segmentation with inaccurate labels.
Shan et al. \cite{Shan2021} attempted to combat the problem of limited available annotated training data by supporting radiologists with a human-involved-mode-iterations (HIMI) strategy. This strategy accelerates the refinement of automatic annotations and therefore leads to more annotated training data. For segmentation, they presented VB-Net, a modified 3D convolutional neural network that combines V-Net \cite{v-net} and a bottleneck structure. From the CT scans of COVID-19 patients, different structures can be segmented, including lung lobes, lung segments, and infected regions. 

Zhou et al. \cite{Zhou2020} addressed the problem of limited training data by introducing a 2.5D segmentation model with a novel data augmentation method. This data augmentation is used to alleviate the amount of training data. Their model is a fully-automatic, rapid, accurate, and machine-agnostic and it can segment and quantify the infection regions from CT scans from different sources. For the data augmentation, they built a CT scan simulator for COVID-19, by fitting the dynamic changes of real patient data measured at different time points obtaining more data.

These studies are all only able to identify and segment the infected region. Yet, it is important that the networks are able to segment different infection patterns such as consolidation and GGO, as they occur at different stages of infection and give clues to the severity and outcome \cite{Yu2020}, and not only a binary pathology. Fan et al. \cite{Fan2020} proposed a COVID-19 Lung Infection Segmentation Deep Network (Inf-Net) that is able to segment radiological patterns such as GGO and consolidation from CT scans of the lung. To address the lack of labeled data, they presented a semi-supervised segmentation strategy that requires only some labeled CTs and then enables the model to use unlabeled data.

Overall, these studies show that the most frequently addressed problem is the limited availability of annotated training data. All of these networks use static data as input to their models. However, patients often have follow-up scans \cite{Jamaludin} to analyze disease progression, resulting in longitudinal datasets. This additional information could be used to improve segmentation despite limited data \cite{kim2021longitudinal}.

\subsection{Longitudinal segmentation}

Longitudinal medical series consist of data collected from the same patient at different points in time. Longitudinal analysis of a disease is important for monitoring its progression and making a prognosis \cite{brainmri}. It can also be used to track the response to different therapies, facilitating adaptive treatment planning, for example in radiotherapy \cite{kim2021longitudinal,head-and-neck}.

Recently, Deep Learning has been increasingly used to analyze longitudinal clinical variables for predicting disease risk or progression, but there is still a need for Deep Learning methods that effectively extract dynamic information from longitudinal images \cite{Cheng2021}.
Instead of segmenting each image individually, segmentation could be improved by using additional information from the longitudinal data, such as the previous scan of the same patient.
Several studies investigated the use of longitudinal data and how this information can be used to improve the segmentation of medical images \cite{vivanti,Birenbaum2017,denner2020spatiotemporal,Cheng2021}.

Vivanti et al. \cite{vivanti} used longitudinal data for the segmentation of liver tumors in follow-up CT scans. As inputs to the network, they used the reference CT scan, a delineation of the tumors in the reference scan as well as the follow-up CT scan. The outputs are the delineation of the tumors in the follow-up CT scan. However, they did not train their network directly with the longitudinal data but only used the reference scans to define a region of interest (ROI) that served as input to the network.
Birenbaum and Greenspan \cite{Birenbaum2017} were the first to propose the use of a longitudinal network for the diagnosis of multiple sclerosis (MS). They presented multiple longitudinal networks to process longitudinal patches from different views. The Siamese architecture contains two separate encoders that share weights. The model then concatenates the encoders' outputs to create a segmentation of MS lesions. This is also known as a late-fusion model \cite{denner2020spatiotemporal}.
Their method shows that incorporating information from multiple time points can be beneficial to the model.

However, these studies do not sufficiently utilize the benefits of learning from structural changes \cite{denner2020spatiotemporal}. 
This additional information could improve segmentation \cite{head-and-neck}, as temporal dynamics between longitudinal scans are more informative than static observations \cite{brainmri}.
The study by Denner et al. \cite{denner2020spatiotemporal} took advantage of this longitudinal information between two scans from two different time points to improve the segmentation of MS lesions. They used in comparison to  \cite{Birenbaum2017} an early fusion network. Here, scans from two time points are concatenated directly and used as input to the network to implicitly encode the structural differences between them. 

Vandewinckele et al. \cite{head-and-neck} proposed an automatic organ at risk (OAR) segmentation network in patients' follow-up images combining deformable image registration and convolutional neural networks. As input to their model, they used the registered longitudinal images, the registered segmentation map of the reference scan, and a segmentation map for the current scan obtained by a separately trained cross-sectional CNN. They decided to train a non-longitudinal cross-sectional CNN to learn relevant intensity features, as the amount of available longitudinal data was very limited.

Recently, there have also been some studies investigating the use of longitudinal chest CT scans to improve segmentation of COVID-19 lesions \cite{foo2021interactive} \cite{kim2021longitudinal}.
Foo et al. \cite{foo2021interactive} used the model of Denner et al. \cite{denner2020spatiotemporal} as a basis and proposed an interactive segmentation method that segments COVID-19 infection on longitudinal CT scans and makes full use of all available past information. In the first round of segmentation, the model takes 3D volumes from two time points as concatenated layers with the additional segmentation of the reference time point as a guide to segment the target scan. In subsequent rounds of segmentation refinement, additional user feedback is fed into the model to correct the segmentation.

Kim et al. \cite{kim2021longitudinal} presented a framework that uses spatio-temporal cues between longitudinal scans to improve quantitative assessment of COVID-19 infection progression. Two concatenated CT scans of a patient were used as input to the model, one reference and one follow-up scan. A 2.5D approach was used, where the model is trained on 2D images for all three views (coronal, sagittal, and axial) and then the predicted probability for a given voxel is averaged over the views. The goal of the model is to segment the follow-up scan into four distinct classes (healthy lung, consolidation, GGO, and pleural effusion). This longitudinal approach showed significant performance improvements compared to a static model. The authors' explanation for this is that the longitudinal images contain the same structural information but differ in the progression of infection. These spatio-temporal cues between the longitudinal scans can be used by the model to improve the segmentation of the follow-up scan.
However, this study has some limitations, such as the very small dataset used for training and evaluation resulting in poor segmentation performance for consolidation and GGO. 


\subsection{Self-supervised pretraining}
\label{section:self-supervised}
To train deep learning-based neural networks, the availability of a large
amount of labeled data is crucial. Manual labeling of image data is expensive and
time-consuming. For natural images, crowdsourcing can be used to obtain labels as no expert knowledge is required \cite{crowd}. However, for medical images, an expert is required to label the data, which makes it hard to obtain large amounts of labeled medical images. Therefore, in general, but especially in the medical field, it is much easier to obtain a large number of unlabeled images \cite{context_restoration}. Boosting the performance of machine learning models by using unlabeled as well as labeled data is an important but challenging problem for which self-supervised learning is a possible solution.

Self-supervised learning is a machine learning strategy that has gained popularity in recent years. It is a new paradigm of unsupervised learning that enables supervised feature learning without the need for labels \cite{context_restoration} \cite{pseudo_lesion}. The supervision tasks are generated from the data itself \cite{pseudo_lesion}. These self-supervision tasks are also called pretext tasks. As a result, a very large number of training instances with supervision are available. Pretraining a CNN using self-supervision results in useful weights for initializing the CNN for the actual target task, for example, segmentation.
Self-supervised pretraining is therefore composed of two steps. First, a CNN is pretraining on a manually designed pretext task with a large amount of unlabeled data. Second, the pretrained network is fine-tuned with a small labeled dataset for the target task. Exploring a large amount of unlabeled data extracts useful information and is a good option to improve the performance of the target task. The main challenge in self-supervised learning is to find a suitable pretext task \cite{context_restoration}\cite{pseudo_lesion}.

The first self-supervision tasks were mainly proposed for natural images \cite{Doersch_2015_ICCV}, \cite{Pathak_2016_CVPR}.
Doersch et al. \cite{Doersch_2015_ICCV} developed a self-supervised learning method to predict the relative position between two patches. For this, a 3x3 field grid is placed over the image and two patches are selected, the central one and one of the surrounding patches. A convolutional neural network is then trained to predict the relative position of the second patch in relation to the central patch.  To perform well on this task, the model must learn to recognize objects and their parts. 

Pathak et al. \cite{Pathak_2016_CVPR} proposed Context Encoders, a context-based pixel prediction. To this end, they trained a convolutional neural network using as input an image in which one or more regions are missing, i.e. set to zero. The network then outputs the missing regions in the input image. To generate the content of these image regions depending, the network has to regress to the missing pixel values based on the environment. 
The masked original image then serves as ground truth. Three different strategies were presented for modifying the input images. Central Region removes a central square patch from the image. Random Block removes several small patches and Random Region removes arbitrary shapes at random locations from the images. Random Region and Random Block were shown to learn general features, significantly outperforming Central Region. They also found that reconstruction loss in conjunction with adversarial loss led to a much sharper result. Context Encoders learn a representation that captures the appearance as well as the semantics of visual structures. It showed effectiveness for CNN pretraining in classification, recognition, and segmentation tasks.

%difference natural and mecial images
Natural images and medical images differ in their intensity distribution. Therefore, pretrained models from the field of natural images are not the optimal choice in the field of medical imaging \cite{context_restoration}. Some studies have therefore investigated self-supervised pretraining using medical images \cite{model_genesis}, \cite{context_restoration}, \cite{pseudo_lesion}.

Zhou et al. \cite{model_genesis} proposed a genesis model to learn robust representations by recovering 3D image patches from a set of transformations. They presented a unified self-supervised learning framework that combines four novel transformations into a single image restoration task. The first transformation is non-linear that uses a smooth and monotonous transformation assigning a unique value to each pixel. It takes advantage of the fact that absolute and relative intensity values in medical images provide important information about the structures and organs. By restoring image patches that have been distorted by a non-linear, the model focuses on learning the appearance of organs. 
The second transformation is local pixel shuffling. This involves sampling a random window and reshuffling the pixels it contains. By restoring the original window, the model must memorize boundaries and texture.
The last two transformations are out-painting and in-painting. Here, an arbitrary number of windows of different sizes are superimposed on top of each other to create a single new window with a complex shape. For out-painting, a random value is assigned to all pixels outside this window, for in-painting to the inner pixels. Through reconstruction, the model learns the context.
These transformations are applied to the random cutout of an unlabeled image. The maximum number of transformations is three, whereby out-painting and in-painting are mutually exclusive. 

The self-supervised learning method of Chen et al. \cite{context_restoration} is based on context restoration of a transformed image. For the transformation, two small random patches are selected from the image, and then their positions are swapped. This process is repeated several times, changing the spatial information but preserving the intensity distribution. A convolutional neural network is then trained to reconstruct the original image. This way, the model learns useful semantic features. A network trained with context restoration leads to improved performance in various tasks such as classification, localization, and segmentation.

Although there is some research on self-supervised learning for medical image data, it has not been extensively used to improve COVID-19 lesion segmentation. In the study by Li et al. \cite{pseudo_lesion}, a novel self-supervised learning method called pseudo-lesion was proposed. The task is specifically designed for COVID-19 CT images and is based on pseudo-lesion generation and restoration.
They used Perlin noise, a gradient noise-based mathematical model, to generate patterns that look like GGO lesions. Patches of these pseudo-lesion patterns are randomly placed on the lung area in clean lung CT scans, generating pseudo-COVID-19 images. The network was trained to remove the pseudo-lesions and reconstruct the clean lung CT. This self-supervised pretraining step improved the performance of a classification algorithm for COVID-19 diagnosis. However, the pretraining was not tested for segmentation.

All of these self-supervised learning tasks are designed for static data and do not consider longitudinal data. Some studies use longitudinal data for self-supervised learning, but none of them use this training to pretrain a longitudinal segmentation network \cite{antoine2019}, \cite{ZHAO2021102051}, \cite{Jamaludin}. Furthermore, there are very few studies that tried to use self-supervised learning to improve COVID-19 segmentation \cite{Fung2021}.

